Secant varieties of toric varieties arising from simplicial complexes

Motivated by the study of the secant variety of the Segre-Veronese variety we propose a general framework to analyze properties of the secant varieties of toric embeddings of affine spaces defined by simplicial complexes. We prove that every such secant is toric, which gives a way to use combinatorial tools to study singularities. We focus on the Segre-Veronese variety for which we completely classify their secants that give Gorenstein or $\mathbb Q$-Gorenstein varieties. We conclude providing the explicit description of the singular locus.

==> 5_figures.tex <==
\section{Figures}




\textcolor{blue}{Example 3.7 (1)\\
	Possibility I, by using the package "tikz"}

\begin{tikzpicture}[x  = {(-0.5cm,-0.5cm)},
y  = {(0.9659cm,-0.25882cm)},
z  = {(0cm,1cm)},
scale = 2]   
\draw[ultra thick,->] (0,0,0) -- (1,0,0);
\draw[ultra thick,->] (0,0,0) -- (0,1,0);
\draw[ultra thick,->] (0,0,0) -- (0,0,1);    
\draw[fill=blue,opacity=0.5] (1,1,0)-- (1,2,0)-- (1,0,2) --(1,0,1)--cycle;
\draw[fill=red,opacity=0.5] (1,1,0)-- (1,2,0)-- (0,2,0)-- cycle;
\draw[fill=orange,opacity=0.5] (1,2,0) --(0,2,0) --(0,0,2)--(1,0,2) --cycle;
\draw[fill=yellow,opacity=0.5] (0,2,0) --(0,0,2) --(1,0,1) --(1,1,0)-- cycle;
\draw[fill=green,opacity=0.5] (0,0,2)-- (1,0,2)-- (1,0,1)-- cycle;      
\end{tikzpicture}   

 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\textcolor{blue}{Example 3.7 (1)\\
	Possibility II, by using the package "pgfplots"}


\begin{tikzpicture}
\begin{axis}[view={105}{30}]
\addplot3[fill=blue,opacity=0.5] coordinates{(1,1,0) (1,2,0) (1,0,2) (1,0,1) (1,1,0)};
\addplot3[fill=red,opacity=0.5] coordinates {(1,1,0) (1,2,0) (0,2,0) (1,1,0)};
\addplot3[fill=orange,opacity=0.5] coordinates {(1,2,0) (0,2,0) (0,0,2) (1,0,2) (1,2,0)};
\addplot3[fill=yellow,opacity=0.5] coordinates {(0,2,0) (0,0,2) (1,0,1) (1,1,0) (0,2,0)};
\addplot3[fill=green,opacity=0.5] coordinates {(0,0,2) (1,0,2) (1,0,1) (0,0,2)};
\end{axis}

\end{tikzpicture}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

 \textcolor{blue}{Example 3.7 (2)\\
	Possibility I, by using the package "tikz"}

\begin{tikzpicture}[x  = {(-0.5cm,-0.5cm)},
y  = {(0.9659cm,-0.25882cm)},
z  = {(0cm,1cm)},
scale = 2]   
\draw[ultra thick,->] (0,0,0) -- (1,0,0);
\draw[ultra thick,->] (0,0,0) -- (0,1,0);
\draw[ultra thick,->] (0,0,0) -- (0,0,1);    
\draw[fill=blue,opacity=0.5] (1,0,2)-- (1,0,1)-- (0,1,1) --(0,1,2)--cycle;
\draw[fill=red,opacity=0.5] (0,1,2)-- (0,0,2)-- (0,1,1)-- cycle;
\draw[fill=orange,opacity=0.5] (0,1,1) --(0,0,2) --(1,0,1) --cycle;
\draw[fill=yellow,opacity=0.5] (1,0,1) --(0,0,2) --(1,0,2)-- cycle;
\draw[fill=green,opacity=0.5] (1,0,2)-- (0,1,2)-- (0,0,2)-- cycle;      
\end{tikzpicture}  

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textcolor{blue}{Example 3.7 (2)\\
	Possibility II, by using the package "pgfplots"}


\begin{tikzpicture}
\begin{axis}[view={105}{30}]
\addplot3[fill=blue,opacity=0.5] coordinates{(1,0,2) (1,0,1) (0,1,1) (0,1,2) (1,0,2)};
\addplot3[fill=red,opacity=0.5] coordinates {(0,1,2) (0,0,2) (0,1,1) (0,1,2)};
\addplot3[fill=orange,opacity=0.5] coordinates {(0,1,1) (0,0,2) (1,0,1) (0,1,1)};
\addplot3[fill=yellow,opacity=0.5] coordinates {(1,0,1) (0,0,2) (1,0,2) (1,0,1)};
\addplot3[fill=green,opacity=0.5] coordinates {(1,0,2) (0,1,2) (0,0,2) (1,0,2)};
\end{axis}

\end{tikzpicture}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textcolor{blue}{Example 3.7 (3)\\
	Possibility I, by using the package "tikz"}

\begin{tikzpicture}[x  = {(-0.5cm,-0.5cm)},
y  = {(0.9659cm,-0.25882cm)},
z  = {(0cm,1cm)},
scale = 2]   
\draw[ultra thick,->] (0,0,0) -- (1,0,0);
\draw[ultra thick,->] (0,0,0) -- (0,1,0);
\draw[ultra thick,->] (0,0,0) -- (0,0,1);
\draw[fill=brown,opacity=0.5] (3,0,0)--(3,2,0)--(0,2,0)--(2,0,0)-- cycle;    
\draw[fill=blue,opacity=0.5] (3,0,0)-- (3,2,0)-- (3,2,1) --(3,0,1)--cycle;
\draw[fill=red,opacity=0.5] (3,2,0)-- (0,2,0)-- (0,2,1)-- (3,2,1)-- cycle;
\draw[fill=orange,opacity=0.5] (0,2,0) --(0,2,1) --(0,1,1) --cycle;
\draw[fill=yellow,opacity=0.5] (0,2,0) --(0,1,1) --(1,0,1)-- (2,0,0)-- cycle;
\draw[fill=green,opacity=0.5] (1,0,1)-- (3,0,1)-- (3,0,0)-- (2,0,0)-- cycle;      
\end{tikzpicture} 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

\textcolor{blue}{Example 3.7 (2)\\
	Possibility II, by using the package "pgfplots"}


\begin{tikzpicture}
\begin{axis}[view={105}{30}]
\addplot3[fill=brown,opacity=0.5]coordinates{(0,2,0) (0,2,1) (0,1,1) (0,2,0)};
\addplot3[fill=blue,opacity=0.5] coordinates{(3,0,0) (3,2,0) (0,2,0) (2,0,0) (3,0,0)};
\addplot3[fill=red,opacity=0.5] coordinates {(3,0,0) (3,2,0) (3,2,1) (3,0,1) (3,0,0)};
\addplot3[fill=orange,opacity=0.5] coordinates {(3,2,0) (0,2,0) (0,2,1) (3,2,1) (3,2,0)};
\addplot3[fill=yellow,opacity=0.5] coordinates {(0,2,0) (0,1,1) (1,0,1) (2,0,0) (0,2,0)};
\addplot3[fill=green,opacity=0.5] coordinates {(1,0,1) (3,0,1) (3,0,0) (2,0,0) (1,0,1)};
\end{axis}

\end{tikzpicture}



